Teaching Interactive Proofs to Mathematicians

This work discusses an approach to teach to mathematicians the importance and effectiveness of the application of Interactive Theorem Proving tools in their specific fields of interest. The approach aims to motivate the use of such tools through short courses. In particular, it is discussed how, using as case-of-study algebraic notions and properties, the use of the proof assistant Prototype Verification System PVS is promoted to interest mathematicians in the development of their mechanized proofs.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{J. Marcos, W. Neuper and P. Quaresma (Eds.): Theorem Proving Components\\ for Educational Software 2020 (ThEdu'20)\\
EPTCS 328, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.328.1}{10.4204/EPTCS.328.1}}
\pdfoutput=1

